Learning Transferable Features for Implicit Neural Representations

Implicit neural representations (INRs) have demonstrated success in a variety of applications, including inverse problems and neural rendering. An INR is typically trained to capture one signal of interest, resulting in learned neural features that are highly attuned to that signal. Assumed to be less generalizable, we explore the aspect of transferability of such learned neural features for fitting similar signals. We introduce a new INR training framework, STRAINER that learns transferrable features for fitting INRs to new signals from a given distribution, faster and with better reconstruction quality. Owing to the sequential layer-wise affine operations in an INR, we propose to learn transferable representations by sharing initial encoder layers across multiple INRs with independent decoder layers. At test time, the learned encoder representations are transferred as initialization for an otherwise randomly initialized INR. We find STRAINER to yield extremely powerful initialization for fitting images from the same domain and allow for $\approx +10dB$ gain in signal quality early on compared to an untrained INR itself. STRAINER also provides a simple way to encode data-driven priors in INRs. We evaluate STRAINER on multiple in-domain and out-of-domain signal fitting tasks and inverse problems and further provide detailed analysis and discussion on the transferability of STRAINER's features. Our demo can be accessed at https://kushalvyas.github.io/strainer.html .

==> content/5_Limitations/Limitations.tex <==
Due to the encoder layers of \strainer being tuned on data and the later layers being randomly initialized, we have observed occasional instability when fitting to a test signal in the form of PSNR ``drops.'' However, we observe that \strainer usually quickly recovers, and the speedup provided by \strainer outweighs this issue.  
While our work demonstrates that INR parameters may be transferred across signals, it is not fully clear what features are being transferred, how they change for different image distributions, and how they compare to the transfer learning of CNNs and Transformers. Further work is needed to characterize these. 



==> content/Motivation/motivation.tex <==
A natural extension to similarity exhibited across signals like natural images is to wonder whether their respective implicit neural representations also showcase such similarity. First, we interpret an INR as a function that progressively warps the input space per layer and fits a given signal through layer wise affine transforms followed by a non linearity \cite{humayun2023splinecam}. While this assumption holds for continuous piecewise affine activation functions, we use an approximation method to visualize (see \Cref{fig:partitions}) the deep network's partition geometry for  different pre-activation level sets \cite{humayun2024deep}. An INR fit to a signal highly adapts to the underlying structure of the data in a layer-wise fashion. Furthermore, 
by approximating the spatial position of the pre-activation zero level sets, we see that initial layers showcase a coarse less-partitioned structure while deeper layers of the network induce dense input space partitioning collocated with sharp changes in the image. Since signals such as natural images tend to show more similarity in their lower frequencies, we therefore propose that initial layers of multiple INRs can be made \emph{transferrable}. We motivate \strainer to share the initial \textit{encoder} layers as multiple INRs fit their respective signals, effectively giving rise to an input space partition that can generalize well across different similar signals.
